Learning to Predict Scene-Level Implicit 3D from Posed RGBD Data

We introduce a method that can learn to predict scene-level implicit functions for 3D reconstruction from posed RGBD data. At test time, our system maps a previously unseen RGB image to a 3D reconstruction of a scene via implicit functions. While implicit functions for 3D reconstruction have often been tied to meshes, we show that we can train one using only a set of posed RGBD images. This setting may help 3D reconstruction unlock the sea of accelerometer+RGBD data that is coming with new phones. Our system, D2-DRDF, can match and sometimes outperform current methods that use mesh supervision and shows better robustness to sparse data.

==> sections/experiments_old.tex <==
\clearpage


We evaluate our method on a two indoor scene dataset of posed RGDB image scans. In this section we evaluate three important claims of our approach a) show we are comparable to using mesh supervision b) perform well against sparse posed depth data c) our learned prior is useful when optimizing for single scenes. Our method needs access to posed RGBD dataset to train but our baselines use mesh supervision we use a real dataset like \matterport and \taskonomy. These datasets provide us reconstructed surfaces (from poisson \nknote{check matterport} reconstruction) along with posed RGBD data. 

We evaluate for each of three settings the methods ability to reconstruct the full 3D scene by using standard metrics and the ray based metric proposed by in DRDF\cite{kulkarni2022s}. We use the ground-truth mesh on the  Below we discuss a short summary of the metrics.
\parnobf{Metrics} We use two primary metrics to capture different aspects of the 3D scene reconstruction task. One metric evaluates completes scenes, and other evaluates individual intersections along a ray by computing the Acc/Cmp/F1score.
\parnoit{Scene Acc/Cmp/F1}. This metric computes the scene-level reconstruction quality by sampling 10K points from the predicted reconstruction and requires ground truth mesh for evaluation. Acc is the percentage of predicted points within a threshold $t=0.5$ of the ground truth mesh. Cmp is the percentage of ground truth points (we sample 10K points on the mesh) are within  a threshold $t=0.5$ of the predicted point cloud.

\parnoit{Ray Acc/Cmp/F1}. This metric evaluates the quality of predicted intersections along a given ray. It computes the Acc and Cmp at $t=0.5$ between ground truth intersection with the 3D mesh and its predicted intersections. We compute this metric for the occluded set of predicted and the ground truth intersections (by dropping the first intersection along the ray). In the main paper we only show results on the occluded intersection  and provide full evaluation in the supplement. We refer to DRDF\cite{kulkarni2022scene} for further details. 

\subsection{How well does \ours fair compared to mesh based methods?}
The foremost thing we evaluate the quality of our reconstruction when training on the full dataset. We compare against baselines that train with full mesh supervision which much more global than our posed RGBD supervision. We primarily compare with DRDF, the best performing method from ~\cite{kulkarni2022scene}. To put our results in context we report the number reported by DRDF baselines as well namely, LDI, UDF, URDF, and ORF.  We additionaly also implement a density based implicit function motivated by PixelNeRF~\cite{yu2020pixelnerf}. All baselines using the same backbone architecture for fair comparison, and we discuss their key ideas below.
% \parnobf{Baselines} We compare against baselines that train with mesh supervision like LDI~\cite{shade1998layered}, DRDF~\cite{kulkarni2022scene} (along with other formulations of distance functions). These methods requires access to explicit 3D geometry (in this case the mesh) to compute the supervisory signal.  We also compare against a PixelNeRF~\cite{yu2020pixelnerf} that is trained to predict the complete 3D of the scene from a single input image while being supervised to predict the 3D geometry using the depth supervision from multiple views. 

\parnoit{\mpd\cite{shade1998layered}} A simple baseline that predicts 4 values for every pixel in the input image. The first value corresponds to the depth of the scene and the rest 3 represent the occluded intersections in the scene. 

\parnoit{\udf \& \urdf \cite{chibane2020ndf}}. Motivated by \cite{chibane2020ndf} this is a fully supervised version of unsigned distance function and the unsigned ray distance function. 

\parnoit{DRDF~\cite{kulkarni2022scene}} This is the fully supervised version of the DRDF function trained with mesh supervision to help us guage the performance gap between RGBD supervision and mesh supervision.

\parnoit{PixelNerf~\cite{yu2020pixelnerf}}  To test the value of predicting a DRDF function as compared to just predicting a density field like in ~\cite{yu2020pixelnerf} we adapt their method to our setting. Their approach allows to predict neural radiance fields for novel unseen images. We modify the implementation from ~\cite{qian2021recognizing} to allows us to train with a single reference view as input and multiple auxiliary views for supervision. In addition to PixelNerf's~\cite{yu2020pixelnerf} color loss when rendered from auxiliary views we supervise the network to also match the ground truth depth from auxiliary views as in \cite{deng2022depth}. At inference, given a single image we predict a feature volume and use an MLP to predict per point density in 3D space. We then convert the  complete density field and decode it to a set of intersections by  integrating along the ray like in \cite{deng2022depth}. This baseline does not use mesh supervision at training and requires the same posed RGBD data as our method.

\parnobf{Datasets}. We compare against baselines on the Matterport3D dataset and use the splits from \cite{kulkarni2022scene}. The full matterport3D dataset consists of 90 scenes split into train/val/test (60/15/15) splits. We consider 15K/1K/1K images from training after filtering images that are has 60\%  of pixel depth values within 1m (images too close to the scene). In total the dataset contains 

\parnobf{Results} We use the results reported by \cite{kulkarni2022scene} in their paper and evaluate. Our method outperforms all the baselines that train with mesh supervision on Scene based metrics. On the ray based metric we show that our method is second best on F1 score when compared to mesh supervised DRDF. This goes to show that our learning signal is equally strong as DRDF's learning signal 

\subsection{How well does \ours work compared to using mesh supervision?}
Our goal is to learn a full 3D scene reconstruction method by using  on RGBD Dataset. We wish to show that our method is robust to sparse data and out performance does not degrade with less number of views. 

\parnobf{Why is depth supervision accurate?}
The key advantage with using depth supervision is that it does not require creating a mesh, and it handles uncertainty of unknown regions better. DRDF treats the mesh as the exact representation of the scene while this is true for cases where the quality of mesh is high, this assumption fails when training on low quality mesh data, or under scanned regions of space. We try to simulate this scenario by sparsely sampling data from out datasets as described below. We believe that learning over a large dataset of sparse views recovers method that can derived supervision from the raw data itself.

\parnobf{Sub sample Frames} We create subsampled versions of datasets at various levels by dropping various \% of RGBD frames from the dataset and then training our method on that. When we drop frames we ensure that of the left frames 70\% contains images that within $15^{\circ}$ of the level, and 30\% come from the rest. \\
\parnoit{\matterport} We sample \matterport at two levels by keeping 50\%, 25\% of the dataset. Below this value the image size of the dataset is small and leads to over-fitting of networks.\\
\parnoit{\taskonomy} The medium split of this dataset contains 100/20 (train/test) scenes. We apply similar strategy as described earlier to filter out bad images from the dataset. Finally our sampled dataset contains 50K input frames for training and we sample 1.3K images for testing. Since this dataset is large it allows us to test our methods in extreme scenarios. We sub sample \taskonomy at three levels and results when this dataset is subsampled to as low as 3\% frames.

\parnobf{Sub sampling Mesh} To train methods like DRDF fairly we need the mesh that is generated from only using sampled frames in the dataset. Instead we use a original mesh that was provided with the dataset and drop faces from it. Our strategy to drop faces involves checking if at least one vertex of the face is visible in any of the frames of the subsampled dataset. In Figure ~\ref{fig:decimation} we show how the quality of the mesh changes with our sampling strategy. This mesh sampling strategy heavily favours the baselines as the supervisory signal for training is derived from a much higher quality mesh than could ever be reconstructed from the sampled frames. We evaluate the quality of decimated meshes by comparing ratio between the area of the decimated mesh and the original mesh, and show this plot in Fig. ~\ref{fig:decimation}. It is important to note that even at 3\% sampled frames meshes still retain over 69\% of the original mesh in area due to our lenient culling strategy (biased in the favour of baselines).

\parnobf{Results} We show that with only 3\% of image frames corresponding to 69\% of the original mesh out method is able to outperform DRDF. Moreover, as we go from 12.5\% data to 3\% data we can see the precipitous fall in the DRDF's F-score which suggest that DRDF is not robust to errors in mesh creation and only works well when we have at least 86\% of the original mesh available.
\nknote{in the table we should have 3\% and the percentage of mesh, maybe we should also show the percentage of drop}


\subsection{Using \ours as Prior model to recover 3D geometry from few images}
The key idea of our approach is that it work with arbitrary number of posed depth images and does not require the underlying mesh to learn. We use this insight and try to complete the 3D geometry of the scene still from a single image but while accounting for additional auxiliary views when we have access to them. 

We test ability of our model by choosing 300 previously unseen images from the test set along with three corresponding auxiliary frames. We then finetune out model trained on large scale scene data to get a more coherent result that respects the auxiliary view. We finetune our model on each instance of the scene for 500 iterations. 
\nknote{need to add a figure for this?}

Our learned scene priors are better as compared to PixelNeRFs density field prior that is also learned with posed RGBD data. We compare the results on scene based and ray based metrics in Table.



\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{example-image-a}
    \caption{Show decimation and plot}
    \label{fig:decimation}
\end{figure}


%\input{tables/ray_scene_pr}

\input{tables/data_size_pr}
\begin{comment}
\section{Experiments}
Baselines to compare --
{\bf Table 1} 


\begin{itemize}
    \item DRDF with full mesh
    \item RGBD DRDF with all depth images cycled for reference views
\end{itemize}


{\bf Table 2} 

\begin{itemize}
    \item DRDF with fixed nbrs -- by dropping vertices 
    \item MPD with fixed nbrs
    \item RGBD DRDF with fixed nbrs
\end{itemize}


{\bf Datasets}
\begin{itemize}
    \item Matterport3D
    \item ARKitScenes
    \item ScanNet
    \item SunRGBD -- no poses too.
    \item NYUv2 -- no poses avaliable -- Will need to run orb-slam with the depth data.
\end{itemize}

\end{comment}

==> tables/data_size_pr.tex <==


\begin{table}[t]
    \setlength{\tabcolsep}{3pt} 
    
    \centering 
    % \resizebox{
    %         \width
    %       }{!}{
    %\captionof{table}{{\bf Scene Acc/Comp/F1Score}. \matterport (MP3D) metrics reported @0.5, \tdf metrics reported @0.5, and \scannet reported 0.2. All metrics are higher the better  $\uparrow$. \tsdf outperforms all baselines on F1 demonstrating better scene reconstruction performance. Further discussion under \S\ref{sec:results}}
    \caption{{\bf Data Percentage Scene Acc/Comp/F1Score}.}
    \vspace{2mm}
    \label{tab:datapercentscene}
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{ls@{~}s@{~}sr@{~}r@{~}rr@{~}r@{~}rs@{~}s@{~}s} \toprule
    & \multicolumn{3}{s}{\drdf } & \multicolumn{3}{r}{\ours } &  \multicolumn{3}{r}{\ours + BS} \\ 
    Data \%   & Acc & Cmp & F1 & Acc  & Cmp & F1 & Acc  & Cmp & F1  \\ 
    \cmidrule(r){1-1}\cmidrule(r){2-4} \cmidrule(r){5-7}  \cmidrule(r){8-10}
     100 & 74.3 & 71.4 & 71.0 & 73.7  & 73.5 & 72.1 & 0 & 0 & 0  \\
     50 (old) & 73.0 & 67.9 & 68.4  & 66.9 & 76.3 & 68.5 & 0 & 0 & 0\\
     50 (new) & 73.0 & 67.9 & 68.4  & 66.9 & 76.9 & 70.0 & 0 & 0 & 0\\
     25 (old) & 72.1 & 65.6 & 66.8 & 66.8 & 74.0 & 68.7 & 0 & 0 & 0\\
     25 (new) & 72.1 & 65.6 & 66.8 & 64.1 & 80.5 & 70.0 & 0 & 0 & 0\\
     12.5 & 72.0 & 63.8 & 65.6 &  -  & - & - & 73.6 & 71.6 & 70.8\\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    
    \end{table}


  
    \begin{table}[t]
      \setlength{\tabcolsep}{3pt} 
      
      \centering 
      % \resizebox{
      %         \width
      %       }{!}{
      %\captionof{table}{{\bf Scene Acc/Comp/F1Score}. \matterport (MP3D) metrics reported @0.5, \tdf metrics reported @0.5, and \scannet reported 0.2. All metrics are higher the better  $\uparrow$. \tsdf outperforms all baselines on F1 demonstrating better scene reconstruction performance. Further discussion under \S\ref{sec:results}}
      \caption{{\bf Data Percentage Ray Acc/Comp/F1Score}.}
      \vspace{2mm}
      \label{tab:datapercentray}
      \begin{adjustbox}{max width=\linewidth}
      \begin{tabular}{ls@{~}s@{~}sr@{~}r@{~}rr@{~}r@{~}rs@{~}s@{~}s} \toprule
      & \multicolumn{3}{s}{\drdf } & \multicolumn{3}{r}{\ours } & \multicolumn{3}{r}{\ours + BS} \\ 
      Data \%   & Acc & Cmp & F1 & Acc  & Cmp & F1  & Acc  & Cmp & F1  \\ 
      \cmidrule(r){1-1}\cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10}
      100 & 29.9 & 24.6 & 27.0  & 28.2  & 22.6 & 25.1 & 0 & 0 & 0  \\
      50 (old) & 28.4 & 20.2 & 23.6  & 21.8 & 24.2 & 22.9 & 0 & 0 & 0 \\
      50 (new) & 28.4 & 20.2 & 23.6  & 22.4 & 26.8 & 24.4 & 0 & 0 & 0  \\
      25 (old) & 27.3 & 17.3 & 21.2 & 21.4 & 22.1 & 21.7 & 0 & 0 & 0  \\
      25 (new) & 27.3 & 17.3 & 21.2 & 21.4 & 29.7 & 24.9 & 0 & 0 & 0 \\
      12.5 & 26.8 & 13.7 & 18.2 &  -  & - & - & 26.2 & 18.9 & 22.0 \\
      \bottomrule
      \end{tabular}
      \end{adjustbox}
      
      \end{table}


==> tables/ray_scene_pr.tex <==


\begin{table}[t]
    \setlength{\tabcolsep}{3pt} 
    
    \centering 
    % \resizebox{
    %         \width
    %       }{!}{
    %\captionof{table}{{\bf Scene Acc/Comp/F1Score}. \matterport (MP3D) metrics reported @0.5, \tdf metrics reported @0.5, and \scannet reported 0.2. All metrics are higher the better  $\uparrow$. \tsdf outperforms all baselines on F1 demonstrating better scene reconstruction performance. Further discussion under \S\ref{sec:results}}
    \caption{{\bf Scene Acc/Comp/F1Score}.}
    \vspace{2mm}
    \label{tab:scene}
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{ls@{~}s@{~}sr@{~}r@{~}rr@{~}r@{~}r} \toprule
    & \multicolumn{3}{s}{Scene } & \multicolumn{3}{r}{Ray } \\ 
    Method   & Acc & Cmp & F1 & Acc  & Cmp & F1  \\ 
    \cmidrule(r){1-1}\cmidrule(r){2-4} \cmidrule(r){5-7}
      \mpd\cite{shade1998layered}  & 66.2 & 72.4 & 67.4 & 13.9 & 42.8 & 19.3  \\ 
     \udf\cite{chibane2020ndf}  & 58.7 & 76.0 & 64.7 & 15.5 & 23.0 & 16.6  \\ 
     \occ  & 73.4 & 69.4 & 69.6 & 26.2 & 20.5 & 21.6 \\ 
     \urdf\cite{chibane2020ndf}  & 74.5 & 67.1 & 68.7 & 24.9 & 20.6 & 20.7 \\ 
     \drdf   & 75.4 & 72.0 &  71.9 &  28.4 &  30.0 & 27.3 \\ 
     \hline
     \drdf  & 74.3 & 71.4 & 71.0 & 29.9 & 24.6 & 27.0 \\
     \hline
     \ours  & 73.7  & 73.5 & 72.1   & 28.2  & 22.6 & 25.1\\
     PixelNeRF & 45.8 & 80.2 & 57.5 & 24.8 & 14.0 & 17.9 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    
    \end{table}

